Efficient and Accurate Memorable Conversation Model using DPO based on sLLM

In multi-session dialog system, it is essential to continuously update the memory as the session progresses. Simply accumulating memory can make it difficult to focus on the content of the conversation for inference due to the limited input sentence size. Therefore, efficient and accurate conversation model that is capable of managing memory to reflect the conversation history continuously is necessary. This paper presents a conversation model that efficiently manages memory as sessions progress and incorporates this into the model to reflect the conversation history accurately with 3 methodologies: SFT, DPO and DPO with SFT model. Our model using DPO algorithm shows an improvement about 0.0591 of BERTScore in memory accuracy, and the rate of responses reflecting the memory increased as well. Also, response generation performance enhanced about 4.292 in fluency, 3.935 in coherence, and 2.896 in consistency. This paper describes a training method that yields better performance than models with more than twice the parameter size, even when the model size is smaller. Thus, our model demonstrates efficiency not only in terms of accuracy but also in resource utilization.

==> section/experiment_2.tex <==
\section{Experiment}
The specific examples used in the actual experiments are detailed in section \ref{experimental_setting} .
%In the summarization and update experiments, the model was configured with prompts. Examples of the actual experiments conducted are specified in the experimental setting section.


\subsection{Experiment Details}

\subsubsection{Summarization Dataset}
To store dialogue in memory in a suitable summarization format, it is essential to extract speaker information that can be utilized in subsequent sessions. Additionally, to facilitate continuous updates of the summarized information, we structured the summaries into short sentences of 15 words or fewer, making them easier to manage than longer context sentences. To effectively train this approach, we designed prompts to create a dataset for Supervised Fine-Tuning (SFT).

Table \ref{tab:psych_issues} presents the mental disorder categories of clients in the test data.
\begin{table}[h]
\centering
\caption{Mental disorder categories of test data}
% \label{tab:psych_issues}
\begin{tabularx}{\columnwidth}{Xr}
    \toprule
    \textbf{Mental Disorder of Client} & \textbf{Number of Cases} \\
    \midrule
    Depression          & 34              \\
    Anxiety             & 22              \\
    Anger Management    & 8               \\
    Trauma              & 6               \\
    \bottomrule
\end{tabularx}
\end{table}

\subsubsection{DPO negative sample}
To apply Direct Preference Optimization (DPO), it is necessary to have pairs of negative and positive samples consisting of rejected and selected samples. The reason for applying DPO in this paper is to accurately reflect the causal facts in the memory. Previous research has used a method of generating negative samples by altering some entities in given sentences to develop benchmarks for evaluating factuality [10]. Therefore, we used prompts to select sentences that accurately reflect cause and effect, generating suitable negative samples for reinforcement learning.

    % Write diverse alternative sentence that contradicts the original case or result by modifying an entity. \n\n sentence: {sentence}

\begin{boxB}
    Write diverse alternative sentence that contradicts the original case or result by modifying an entity. Sentence: \{sentence\}
\end{boxB}
\noindent The model should generate appropriate utterances in the ``utterance" field. This structured format reduces confusion when the model generates its answer and aids in the post-processing of generated text.


\subsubsection{Metric}
We use Llama2-7B, Llama3-70B as baseline models for generating multi-turn counseling dialogues. We chose these models because they are open-sourced and easily reproducible. We also compare these results with the Llama2-7B model that has been fine-tuned on the Counsel Chat dataset, which is available on HuggingFace \footnote{https://huggingface.co/NadunAnjanaka/Llama-2-7b-chat-Counsellor}.

\begin{boxB}
    $T=\{t1, t2, t3\}, P=\{p1, p2, p3\}, S=\{s1, s2\}$ \newline
    $S1=cosine\_similarity(Tn, Am) \geq  0.7$,\newline
    $S2=BERTScore(Tn, Am) \geq  0.95$ \newline
    Accuracy=n(S1)/n(P) \ or \ n(S2)/n(P)
\end{boxB}


\subsubsection{Experimental setting} \label{experimental_setting}
%We evaluate two experimental settings: 1) zero-shot multi-turn dialogue generation, 2) few-shot multi-turn dialogue generation.
We evaluate two experimental settings: 1) zero-shot multi-turn dialogue generation (see Figure \ref{fig:zero-shot_example} for example), 2) few-shot multi-turn dialogue generation (see Figure \ref{fig:few-shot_example} for example). Results are compared within the same mental disorder category. We consider these settings because well-constructed synthetic multi-turn counseling data should improve the model's few-shot dialogue generation capabilities.

\begin{figure}[ht]
  \centering
  \begin{boxB}
        The following is a transcript of a chat between a psychotherapist and a client about depression.
        The client starts the conversation as [client] and the psychotherapist starts the conversation as [psychotherapist]. Please complete new transcript about [Question].\newline\newline
        [Question] \newline
        [client] I'm almost never happy. Half of the time, I don't feel anything. I find it easy to make myself feel nothing. I know I push people away because it’s easier. I just want answers. I'm sick of feeling this way. It’s ruining my relationships with people. \newline
        [psychotherapist]
    \end{boxB}
  \caption{Example of zero-shot prompt}
  \label{fig:zero-shot_example}
\end{figure}

\begin{figure}[ht!]
  \centering
  \begin{boxB}
        The following is a transcript of a chat between a psychotherapist and a client about depression.
        The client starts the conversation as [client] and the psychotherapist starts the conversation as [psychotherapist].
        Please use the following [Example] as a guide complete new transcript about [Question].\newline\newline
        [Example] \newline
        [client] They don't go away, and I feel like I'm going crazy. Does that ever stop? Can it be a symptom of medication?\newline
        [psychotherapist] Since you realize that hearing voices in your head is not usual for you, then definitely there is a problematic situation happening within your awareness of who you are.if you recently started taking a new drug or increased dosage of one you already were taking, and the voices started shortly after, then yes, it is possible medication created your problem.Start by telling whoever gave you the presecription, about the problem you\'re having."Crazy" has some flexibility as to whether someone is this way or not.Certainly a very positive sign that you\'re not crazy, is that you\'re self-aware of a problem within yourself. And, you\'re responsible toward yourself and making effort to address this problem.Crazy people usually don\'t do responsible behaviors.\newline
        [client] I've been taking the same medication for a while now, but the dosage was increased a few weeks ago. Could that be the cause of the voices?\newline
        [psychotherapist] That's a good point. The dosage increase could definitely be a contributing factor. It's possible that your body is reacting to the higher dosage in a way that's causing these symptoms. I would still recommend reporting this to your prescribing doctor, as they can help you determine the best course of action. \newline
        \newline
        [Question]\newline
        [client] I have been dealing with depression and anxiety for a number of years. I have been on medication, but lately my depression has felt worse. Can counseling help? \newline
        [psychotherapist]
    \end{boxB}
  \caption{Example of few-shot prompt}
  \label{fig:few-shot_example}
\end{figure}


\subsubsection{Automatic Evaluation}
We conduct an automatic evaluation using GPT-4o, the latest model introduced by OpenAI. The evaluation prompt is described in Figure \ref{fig:geval_example}

\begin{figure}[ht!]
  \centering
  \begin{boxB}
    You're an assistant who evaluates answers strictly from the psychotherapist's perspective about \{mental disorder category\}. Please rate [Answer 1] and [Answer 2] for the consultation [Question], respectively. Rate the two answers on a scale of 1-5, with higher values indicating better answers.
  \end{boxB}
  \caption{Example of evaluation prompt}
  \label{fig:geval_example}
\end{figure}


\noindent We follow the G-Eval methodology \cite{liu2023geval} for conducting automatic evaluations.

% 평가 점수 넣기
\subsection{Result}

\subsubsection{Evaluation of Zero-shot and Few-shot Performance}
%\subsubsection{Evaluation of Zero-shot and Few-shot Performance}

%70B를 제외하고 7B에서 비교한 내용만 적혀져야 함, 여기에 counselor data로 학습한 llama2-chat-counselor 모델과의 비교도 적혀져야 함
Table \ref{tab:avg_win_counts} presents the average scores evaluated by GPT-4o for the two models, Llama2-7B-Chat and Llama3-70B-Instruct, in zero-shot and few-shot settings. The average score in the zero-shot category is 3.814 for Llama2-7B-Chat, slightly lower than the 4.042 for Llama3-70B-Instruct, indicating marginally better performance by Llama3-70B-Instruct when no prior examples are provided.
In the few-shot setting, Llama2-7B-Chat has an average score of 4.557, while Llama3-70B-Instruct achieves 4.785, demonstrating that both models perform better when examples generated by our pipeline are provided.

% Table \ref{tab:avg_win_counts} presents the average win counts for two models, Llama2-7B-Chat and Llama3-70B-Instruct, for zero-shot and few-shot performance. The average win count in the zero-shot category is 3.814 for Llama2-7B-Chat and slightly higher at 4.042 for Llama3-70B-Instruct, indicating that Llama3-70B-Instruct performs marginally better when no prior examples are provided. In the few-shot setting, the average win count is 4.557 for Llama2-7B-Chat and 4.785 for Llama3-70B-Instruct, showing that both models achieve better performance when examples generated by our pipeline are provided.


\begin{table}[h]
\centering
\caption{Average evaluation score evaluated by GPT-4o}
\label{tab:avg_win_counts}
\begin{tabularx}{\columnwidth}{Xrr}
    \toprule
    \textbf{Model} & \textbf{Zeroshot Avg.} & \textbf{Fewshot Avg.} \\
    \midrule
    Llama2-7B-Chat & 3.814 & 4.557 \\
    Llama2-70B-Instruct & 4.042 & 4.785 \\
    \bottomrule
\end{tabularx}
\end{table}



\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figure/win_zzin_final.png}
  \caption{Comparison of zero-shot and few-shot multi-turn counseling dialogue generation performance for Llama2-7B-chat and Llama3-70B-Instruct. In the few-shot setting, examples generated by our pipeline are used.}
  \label{fig:win}
\end{figure}

Figure \ref{fig:win} compares the win rates of two models, Llama2-7B-chat and Llama3-70B-Instruct, in terms of their few-shot multi-turn generation performance. Zero-shot wins are shown in green, few-shot wins in peach, and ties in light grey. Each count reflects the win rate comparison between the two models' zero-shot and few-shot capabilities. Llama2-7B-chat recorded 14 zero-shot wins, 55 few-shot wins, and 1 Tie. Llama3-70B-Instruct, on the other hand, had 11 zero-shot wins, 56 few-shot wins, and 3 ties. The results suggest that Llama3-70B-Instruct performs slightly better in few-shot multi-turn generation. In both Llama2 and Llama3 model, using few-shot examples constructed by our pipeline contributes to generating better quality of multi-turn counseling conversation. Using few-shot examples constructed by our pipeline enhances the models' ability to generate high-quality multi-turn counseling conversations in both Llama2 and Llama3.


\subsubsection{Evaluation of Zero-shot and Few-shot Performance based on Mental Disorder Categories}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figure/win_category_final.png}
  \caption{Comparison of zero-shot and few-shot multi-turn counseling dialogue generation performance across mental disorder categories for Llama2-7B-Chat and Llama3-70B-Instruct.}
  \label{fig:win_category}
\end{figure}


Figure \ref{fig:win_category} shows a comparative analysis of win counts by category for Llama2-7B-Chat (upper) and Llama3-70B-Instruct (lower). Win counts are categorized into zero-shot (green), few-shot (peach), and tie (grey) for mental disorders including Depression, Anxiety, Anger-management, and Trauma.
Llama2-7B-Chat demonstrates the highest win counts in the few-shot category, with 28 wins in Depression and 15 in Anxiety. Similarly, Llama3-70B-Instruct shows robust few-shot performance, recording 27 wins in Depression and 18 in Anxiety.
This comparison shows that both models are particularly effective in few-shot scenarios across all disorders. 
The overall trend highlights the superior performance of few-shot dialogue generation for both models in addressing various psychological disorders.

\subsubsection{Evaluation of Performance Based on Data Used}

\begin{table}[h]
\centering
\caption{Win rate and average evaluation score evaluated by GPT-4o}
\label{tab:data_perform}
\begin{tabularx}{\columnwidth}{Xrr}
    \toprule
    \textbf{Model} & \textbf{Win rate} & \textbf{Avg.} \\
    \midrule
    Llama2-7B-Chat-Counsellor\cite{bertagnolli2020counsel} & 0.014 & 1.828 \\
    Llama2-7B-Chat Few-shot & 0.985 & 4.528 \\
    \bottomrule
\end{tabularx}
\end{table}

The experimental setup involved comparing Llama2-7B-Chat-Counsellor and Llama2-7B-Chat Few-shot, with the results illustrated in Table \ref{tab:data_perform}.

Table \ref{tab:data_perform} demonstrates a clear comparison between the two models' performance. Llama2-7B-Chat-Counsellor achieved an average score of 1.828, while Llama2-7B-Chat Few-shot significantly outperformed Llama2-7B-Chat-Counsellor with an average score of 4.528. These results indicate that Llama2-7B-Chat Few-shot is markedly more effective in generating high-quality, contextually appropriate, and supportive responses in extended multi-turn interactions compared to Llama2-7B-Chat-Counsellor.

This substantial difference in average scores underscores the effectiveness of the pipeline proposed in our research for transforming single-turn data into high-quality multi-turn datasets. The enhanced performance of Llama2-7B-Chat Few-shot suggests that the comprehensive approach we employed, which includes collecting detailed information from both counselors and clients and incorporating data on various mental health disorders, is crucial for improving the capabilities of LLMs in psychological counseling scenarios.

% \section{Dataset Analysis}

% figure
%% pipeline 1
%% data prompt (extraction info, multi-turn 구축)
%% figure - evaluation (win rate)

% evaluation pipeline - zero shot, few shot evaluation

==> section/method_ysh_kor.tex <==
% 문제: Recursively 논문도 memory management 모듈이라는 이름을 있음. 
% 차이점: 
%  - 성능 관점: 1) DPO, 학습 효율, 
%            2) Memory Update 정확도 개선 + generation 성능 개선 
%  - 메모리 관리 전략: 복합 문장의 생성 요약 기반의 메모리 관리 X 
%               ==> 모니터링/해석성이 용이한 단문 형태의 대화 히스토리 관리 
% 정리하면, DPO를 하는 이유는 크게 두가지가 있음: 첫째는 학습 효율과 생성 문장의 정확도 측면. 둘째는 더 효과적인 메모리 효과 전략.
% Consequences: 
%   1) LLAMA3-8B보다 더 우월한 멀티 세션 대화에서의 생성 성능을 확보 
%   2) 기존 Recursively 방법보다 약간의 데이터 구축 및 학습 과정이라는 tradeoff가 있지만, 더 정확도 있는 요약문 업데이트 및 답변 생성이 가능함. (실험적으로 입증) 

== 

%메모리 모듈- 메모리 관리 모듈은 마지막 대화 세션에서 나타난 화자의 발화 정보들을 미래의 새로운 대화 세션에 참고하기 위해 별도의 메모리 공간에 저장하는 것을 주된 목적으로 한다. 이 모듈은 매번 대화 세션이 종료된 직후에 이전 대화 세션까지 업데이트 된 메모리의 화자 정보를 바탕으로 현재 대화 세션의 내용을 참조하여 메모리를 업데이트 합니다. 이를 위해 우리는 DPO 알고리즘을 이용하여 튜닝된 SLM을 활용한 요약 기반의 대화 히스토리 관리 방법을 제안한다. 제안 방법은 화자 발화의 핵심 정보들을 단문 형태의 집합으로 관리할 수 있게 한다. 제안 방벙은 생성 답변의 정확도 개선과 학습 효율의 극대화 그리고 단문 형태의 화자 정보 관리를 통해 모니터링이 용이하다는 장점을 가지고 있다. 

%두번째 대화 생성 모듈은 현재 세션 대화 맥락 뿐만 아니라 이전 대화 세션의 정보도 효과적으로 반영하여 사용자에게 더 일관성있고 정확도 높은 생성 답변을 목적으로 한다. As shown in Figure \ref{fig:main_figure}, 대화 생성 모듈은 N-1번째 대화 세션까지 업데이트된 메모리의 정보를 입력 프롬프트로 전달받는다. 이것은 모듈이 과거 시점에 발생한 대화 히스토리도 적절히 참고할 수 있기 때문에 시간적 차이에서 발생하던 과거의 문제점을 다룰 수 있게 된다. 본 논문에서 우리는 대화 생성 모듈로서 phi-3 모델을 별도의 추가 학습 없이 활용한다. 그 결과 우리는 2배 이상 많은 파라미터를 가진 llama3-8b 모델과 비교했을 때도 더 높은 정확도를 가진 생성 대화 능력을 확인할 수 있었다. 다음은 각 모듈에 대한 상세 설명을 포함하며 특히 본 논문의 차별성인 DPO를 활용한 효과적인 메모리 관리 모듈의 학습 방법을 상세히 설명한다. 





우리는 화자의 발화 내용을 복합 문장 형식의 정리된 요약문 형태의 
% 
%(Dialog Generation에서) 그래서 이것은 새로운 대화 세션이 진행되면 대화 생성 모듈의 프롬프트로 전달된다. 그 결과 대화 생성 모듈은 과거 시점에 발생한 대화 히스토리도 적절히 참고할 수 있게 되며 사용자에게 더 engaging한 대대화 경험을 제공할 수 있게 된다.
%우리는 메모리 관리 모듈로서 3.8B 파라미터를 가진 phi-3모델을 백본으로 사용하며 우리는   
이것은 세션이 진행됨에 따라 핵심 정보들을 누적 관리할 수 있어야 하며, 그 과정에서  
단문 형태의 집합으로 관리하는 것을 목적으로 한다. 
%비교 모델: Recursively Summarize 
%

==> section/preliminary_2.tex <==


\section{Methodology}
\subsection{Task Definition}


\subsubsection{Memory management}
To maximize the utilization of therapist information, we preprocess the source dataset. According to the latest South Korean government report\footnote{\url{https://www.ncmh.go.kr/mentalhealth/main.do}}, which identifies severe stress, continuous depression, anxiety, and sleep disorders, as the most prevalent mental illnesses in 2022, we have selected these conditions as our focus for an augmented dataset.

\subsubsection{Memory update}

\subsubsection{Dialog generation}

%To maximize the utilization of therapist information, we preprocess the source dataset. According to the latest 2022 report by the South Korean government\footnote{\url{https://www.ncmh.go.kr/mentalhealth/main.do}}, severe stress, persistent depression, anxiety, and sleep disorders have been identified as the most common mental health issues. Therefore, we have focused on these conditions in the augmented dataset.


